The Atacama Cosmology Telescope: Modeling Bulk Atmospheric Motion

Fluctuating atmospheric emission is a dominant source of noise for ground-based millimeter-wave observations of the CMB temperature anisotropy at angular scales $\gtrsim 0.5^{\circ}$. We present a model of the atmosphere as a discrete set of emissive turbulent layers that move with respect to the observer with a horizontal wind velocity. After introducing a statistic derived from the time-lag dependent correlation function for detector pairs in an array, referred to as the pair-lag, we use this model to estimate the aggregate angular motion of the atmosphere derived from time-ordered data from the Atacama Cosmology Telescope (ACT). We find that estimates derived from ACT's CMB observations alone agree with those derived from satellite weather data that additionally include a height-dependent horizontal wind velocity and water vapor density. We also explore the dependence of the measured atmospheric noise spectrum on the relative angle between the wind velocity and the telescope scan direction. In particular, we find that varying the scan velocity changes the noise spectrum in a predictable way. Computing the pair-lag statistic opens up new avenues for understanding how atmospheric fluctuations impact measurements of the CMB anisotropy.

==> authors.tex <==

\author{
Thomas~Morris\altaffilmark{3},
%Steve~K.~Choi\altaffilmark{1,2,3},
%Matthew~Hasselfield\altaffilmark{4,5,6},
%Shuay-Pwu~Patty~Ho\altaffilmark{3},
%Brian~Koopman\altaffilmark{7},
%Marius~Lungu\altaffilmark{3,8},
%Maximilian~H.~Abitbol\altaffilmark{9},
%Graeme~E.~Addison\altaffilmark{10},
%Peter~A.~R.~Ade\altaffilmark{11},
%Simone~Aiola\altaffilmark{4,3},
%David~Alonso\altaffilmark{9},
%Mandana~Amiri\altaffilmark{12},
%Stefania~Amodeo\altaffilmark{2},
%Elio~Angile\altaffilmark{8},
%Jason~E.~Austermann\altaffilmark{13},
%Taylor~Baildon\altaffilmark{14},
%Nick~Battaglia\altaffilmark{2},
%James~A.~Beall\altaffilmark{13},
%Rachel~Bean\altaffilmark{2},
%Daniel~T.~Becker\altaffilmark{13},
%J~Richard~Bond\altaffilmark{15},
%Sarah~Marie~Bruno\altaffilmark{3},
Ricardo Bustos, 
Erminia~Calabrese\altaffilmark{11},
%Victoria~Calafut\altaffilmark{2},
%Luis~E.~Campusano\altaffilmark{16},
%Felipe~Carrero\altaffilmark{17},
%Grace~E.~Chesmore\altaffilmark{18},
%Hsiao-mei~Cho.\altaffilmark{19,13},
%Susan~E.~Clark\altaffilmark{20},
%Nicholas~F.~Cothard\altaffilmark{21},
%Devin~Crichton\altaffilmark{22},
%Kevin~T~Crowley\altaffilmark{23,3},
%Omar~Darwish\altaffilmark{24},
%Rahul~Datta\altaffilmark{10},
%Edward~V.~Denison\altaffilmark{13},
%Mark~J.~Devlin\altaffilmark{8},
%Cody~J.~Duell\altaffilmark{1},
%Shannon~M.~Duff\altaffilmark{13},
Adriaan~J.~Duivenvoorden\altaffilmark{3},
Jo~Dunkley\altaffilmark{3,25},
Rolando~D\"{u}nner\altaffilmark{26},
%Thomas~Essinger-Hileman\altaffilmark{27},
%Max~Fankhanel\altaffilmark{17},
%Simone~Ferraro\altaffilmark{28},
%Anna~E.~Fox\altaffilmark{13},
%Brittany~Fuzia\altaffilmark{29},
%Patricio~A.~Gallardo\altaffilmark{1},
%Vera~Gluscevic\altaffilmark{30},
%Joseph~E.~Golec\altaffilmark{18},
%Emily~Grace\altaffilmark{3},
%Megan~Gralla\altaffilmark{31},
%Yilun~Guan\altaffilmark{32},
%Kirsten~Hall\altaffilmark{10},
%Mark~Halpern\altaffilmark{12},
%Dongwon~Han\altaffilmark{33},
%Peter~Hargrave\altaffilmark{11},
%Shawn~Henderson\altaffilmark{19},
%Brandon~Hensley\altaffilmark{25},
%J.~Colin~Hill\altaffilmark{34,4},
%Gene~C.~Hilton\altaffilmark{13},
%Matt~Hilton\altaffilmark{22},
%Adam~D.~Hincks\altaffilmark{35},
%Ren\'ee~Hlo\v{z}ek\altaffilmark{36,35},
%Johannes~Hubmayr\altaffilmark{13},
%Kevin~M.~Huffenberger\altaffilmark{29},
%John~P.~Hughes\altaffilmark{37},
%Leopoldo~Infante\altaffilmark{26},
%Kent~Irwin\altaffilmark{38},
%Rebecca~Jackson\altaffilmark{18},
%Jeff~Klein\altaffilmark{8},
%Kenda~Knowles\altaffilmark{22},
%Arthur~Kosowsky\altaffilmark{32},
%Vincent~Lakey\altaffilmark{29},
%Dale~Li\altaffilmark{19,13},
%Yaqiong~Li\altaffilmark{3},
%Zack~Li\altaffilmark{25},
%Martine~Lokken\altaffilmark{35,15},
%Thibaut~Louis\altaffilmark{39},
%Amanda~MacInnis\altaffilmark{33},
%Mathew~Madhavacheril\altaffilmark{40},
%Felipe~Maldonado\altaffilmark{29},
%Maya~Mallaby-Kay\altaffilmark{41},
%Danica~Marsden\altaffilmark{8},
%Lo\"ic~Maurin\altaffilmark{42,26},
%Jeff~McMahon\altaffilmark{43,41,18,44,14},
%Felipe~Menanteau\altaffilmark{45,46},
%Kavilan~Moodley\altaffilmark{22},
%Tim~Morton\altaffilmark{30},
Sigurd~Naess\altaffilmark{4},
%Toshiya~Namikawa\altaffilmark{24},
%Federico~Nati\altaffilmark{47,8},
%Laura~Newburgh\altaffilmark{7},
%John~P.~Nibarger\altaffilmark{13},
%Andrina~Nicola\altaffilmark{25},
%Michael~D.~Niemack\altaffilmark{1,2},
%Michael~R.~Nolta\altaffilmark{15},
%John~Orlowski-Sherer\altaffilmark{8},
Lyman~A.~Page\altaffilmark{3},
%Christine~G.~Pappas\altaffilmark{13},
Bruce~Partridge\altaffilmark{48},
%Phumlani~Phakathi\altaffilmark{22},
%Heather~Prince\altaffilmark{25},
%Roberto~Puddu\altaffilmark{26},
%Frank~J.~Qu\altaffilmark{24},
%Jesus~Rivera\altaffilmark{37},
%Naomi~Robertson\altaffilmark{49},
%Felipe~Rojas\altaffilmark{26,17},
%Maria~Salatino\altaffilmark{38,50},
%Emmanuel~Schaan\altaffilmark{28},
%Alessandro~Schillaci\altaffilmark{51},
%Benjamin~L.~Schmitt\altaffilmark{8},
%Neelima~Sehgal\altaffilmark{33},
%Blake~D.~Sherwin\altaffilmark{24},
%Carlos~Sierra\altaffilmark{18},
%Jon~Sievers\altaffilmark{52},
%Cristobal~Sifon\altaffilmark{53},
%Precious~Sikhosana\altaffilmark{22},
%Sara~Simon\altaffilmark{14,54},
%David~N.~Spergel\altaffilmark{4,25},
%Suzanne~T.~Staggs\altaffilmark{3},
%Jason~Stevens\altaffilmark{1},
%Emilie~Storer\altaffilmark{3},
%Dhaneshwar~D.~Sunder\altaffilmark{22},
%Eric~R.~Switzer\altaffilmark{27},
%Ben~Thorne\altaffilmark{55},
%Robert~Thornton\altaffilmark{56,8},
%Hy~Trac\altaffilmark{57},
Jesse~Treu\altaffilmark{58},
%Carole~Tucker\altaffilmark{11},
%Leila~R.~Vale\altaffilmark{13},
%Alexander~Van~Engelen\altaffilmark{59},
%Jeff~Van~Lanen\altaffilmark{13},
%Eve~M.~Vavagiakis\altaffilmark{1},
%Kasey~Wagoner\altaffilmark{3},
%Yuhan~Wang\altaffilmark{3},
%Jonathan~T.~Ward\altaffilmark{8},
%Edward~J.~Wollack\altaffilmark{27},
Zhilei~Xu\altaffilmark{8},
%Fernando~Zago\altaffilmark{52},
%Ningfeng~Zhu\altaffilmark{8}
}
%\altaffiltext{1}{Department of Physics, Cornell University, Ithaca, NY, USA %14853}
%\altaffiltext{2}{Department of Astronomy, Cornell University, Ithaca, NY %14853, USA}
\altaffiltext{3}{Joseph Henry Laboratories of Physics, Jadwin Hall,
Princeton University, Princeton, NJ, USA 08544}
\altaffiltext{4}{Center for Computational Astrophysics, Flatiron Institute, 162 5th Avenue, New York, NY 10010 USA}
%\altaffiltext{5}{Department of Astronomy and Astrophysics, The Pennsylvania %State University, University Park, PA 16802, USA}
%\altaffiltext{6}{Institute for Gravitation and the Cosmos, The Pennsylvania %State University, University Park, PA 16802, USA}
%\altaffiltext{7}{Department of Physics, Yale University, 217 Prospect St, %New Haven, CT 06511}
\altaffiltext{8}{MIT Kavli Institute, Massachusetts Institute of Technology, 77 Massachusetts Avenue, Cambridge, MA 02139, USA
ORCID: 0000-0001-5112-2567}
%\altaffiltext{9}{Department of Physics, University of Oxford, Keble Road, %Oxford, UK OX1 3RH}
%\altaffiltext{10}{Dept. of Physics and Astronomy, The Johns Hopkins %University, 3400 N. Charles St., Baltimore, MD, USA 21218-2686}
\altaffiltext{11}{School of Physics and Astronomy, Cardiff University, The Parade, 
Cardiff, Wales, UK CF24 3AA}
%\altaffiltext{12}{Department of Physics and Astronomy, University of
%British Columbia, Vancouver, BC, Canada V6T 1Z4}
%\altaffiltext{13}{NIST Quantum Devices Group, 325
%Broadway Mailcode 817.03, Boulder, CO, USA 80305}
%\altaffiltext{14}{Department of Physics, University of Michigan, Ann Arbor, %USA 48103}
%\altaffiltext{15}{Canadian Institute for Theoretical Astrophysics, %University of
%Toronto, Toronto, ON, Canada M5S 3H8}
%\altaffiltext{16}{Universidad de Chile, Dept Astronom\'{i}a Casilla 36-D, %Santiago, Chile}
%\altaffiltext{17}{Sociedad Radiosky Asesor\'{i}as de Ingenier\'{i}a Limitada %Lincoy\'{a}n 54,
%Depto 805 Concepci\'{o}n, Chile}
%\altaffiltext{18}{Department of Physics, University of Chicago, Chicago, IL %60637, USA}
%\altaffiltext{19}{SLAC National Accelerator Laboratory 2575 Sand Hill Road %Menlo Park, California 94025, USA}
%\altaffiltext{20}{Institute for Advanced Study, 1 Einstein Dr, Princeton, NJ %08540}
%\altaffiltext{21}{Department of Applied and Engineering Physics, Cornell %University, Ithaca, NY, USA 14853}
%\altaffiltext{22}{Astrophysics Research Centre, School of Mathematics, %Statistics and Computer Science, University of KwaZulu-Natal, Durban 4001, %South 
%Africa}
%\altaffiltext{23}{Department of Physics, University of California, Berkeley, %CA, USA 94720}
%\altaffiltext{24}{DAMTP, Centre for Mathematical Sciences, University of %Cambridge, Wilberforce Road, Cambridge CB3 OWA, UK}
\altaffiltext{25}{Department of Astrophysical Sciences, Peyton Hall, 
Princeton University, Princeton, NJ USA 08544}
%\altaffiltext{26}{Instituto de Astrof\'isica and Centro de %Astro-Ingenier\'ia, Facultad de F\`isica, Pontificia Universidad Cat\'olica %de Chile, Av. Vicu\~na Mackenna 4860, 7820436 Macul, Santiago, Chile}
\altaffiltext{27}{NASA/Goddard Space Flight Center, Greenbelt, MD, USA 20771}
%\altaffiltext{28}{Berkeley Center for Cosmological Physics, LBL and
%Department of Physics, University of California, Berkeley, CA, USA 94720}
%\altaffiltext{29}{Department of Physics, Florida State University, %Tallahassee FL, USA 32306}
%\altaffiltext{30}{University of Southern California. Department of Physics %and Astronomy, 825 Bloom Walk ACB 439. Los Angeles, CA 90089-0484}
%\altaffiltext{31}{Department of Astronomy/Steward Observatory, University of %Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065}
%\altaffiltext{32}{Department of Physics and Astronomy, University of %Pittsburgh, 
%Pittsburgh, PA, USA 15260}
%\altaffiltext{33}{Physics and Astronomy Department, Stony Brook University, %Stony Brook, NY USA 11794}
%\altaffiltext{34}{Department of Physics, Columbia University, New York, NY, %USA}
%\altaffiltext{35}{David A. Dunlap Department of Astronomy and Astrophysics, %University of Toronto, 50 St George Street, Toronto ON, M5S 3H4, Canada}
%\altaffiltext{36}{Dunlap Institute for Astronomy and Astrophysics, %University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
%\altaffiltext{37}{Department of Physics and Astronomy, Rutgers, 
%The State University of New Jersey, Piscataway, NJ USA 08854-8019}
%\altaffiltext{38}{Department of Physics, Stanford University, Stanford, CA, 
%USA 94305-4085}
%\altaffiltext{39}{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 %Orsay, France}
%\altaffiltext{40}{Centre for the Universe, Perimeter Institute for %Theoretical Physics, Waterloo, ON, N2L 2Y5, Canada}
%\altaffiltext{41}{Department of Astronomy and Astrophysics, University of %Chicago, 5640 S. Ellis Ave., Chicago, IL 60637, USA}
%\altaffiltext{42}{Universit\'e Paris-Saclay, CNRS, Institut d'astrophysique %spatiale, 91405, Orsay, France.}
%\altaffiltext{43}{Kavli Institute for Cosmological Physics, University of %Chicago, 5640 S. Ellis Ave., Chicago, IL 60637, USA}
%\altaffiltext{44}{Enrico Fermi Institute, University of Chicago, Chicago, IL %60637, USA}
%\altaffiltext{45}{National Center for Supercomputing Applications (NCSA), %University of Illinois at Urbana-Champaign, 1205 W. Clark St., Urbana, IL, %USA, 61801}
%\altaffiltext{46}{Department of Astronomy, University of Illinois at %Urbana-Champaign, W. Green Street, Urbana, IL, USA, 61801}
%\altaffiltext{47}{Department of Physics, University of Milano - Bicocca, %Piazza della Scienza, 3 - 20126, Milano (MI), Italy}
\altaffiltext{48}{Department of Physics and Astronomy, Haverford College,
Haverford, PA, USA 19041}
%\altaffiltext{49}{Institute of Astronomy, Madingley Road, Cambridge CB3 0HA, %UK}
%\altaffiltext{50}{Kavli Institute for Particle Astrophysics and Cosmology, %382 Via Pueblo Mall Stanford, CA  94305-4060, USA}
%\altaffiltext{51}{Department of Physics, California Institute of Technology, %Pasadena, California 91125, USA}
%\altaffiltext{52}{Physics Department, McGill University, Montreal, QC H3A %0G4, Canada}
\altaffiltext{53}{Instituto de F{\'{i}}sica, Pontificia Universidad Cat{\'{o}}lica de Valpara{\'{i}}so, Casilla 4059, Valpara{\'{i}}so, Chile}
%\altaffiltext{54}{Fermi National Accelerator Laboratory, MS209, P.O. Box %500, Batavia, IL 60510}
%\altaffiltext{55}{One Shields Avenue, Physics Department, Davis, CA 95616, %USA}
%\altaffiltext{56}{Department of Physics , West Chester University 
%of Pennsylvania, West Chester, PA, USA 19383}
%\altaffiltext{57}{McWilliams Center for Cosmology, Carnegie Mellon %University, Department of Physics, 5000 Forbes Ave., Pittsburgh PA, USA, %15213}
\altaffiltext{58}{Domain Associates, LLC}
%\altaffiltext{59}{School of Earth and Space Exploration, Arizona State %University, Tempe, AZ, USA 85287}
%\altaffiltext{60}{Department of High Energy Physics, Argonne National %Laboratory, 9700 S Cass Ave, Lemont, IL USA 60439}
%\altaffiltext{61}{Department of Astronomy, University of Chicago, Chicago, %IL USA}
%\altaffiltext{62}{Astrophysics and Cosmology Research Unit, School of %Chemistry and Physics, University of KwaZulu-Natal, Durban 4001, South %Africa}
%\altaffiltext{63}{Kavli Institute for Cosmology Cambridge, Madingley Road, %Cambridge CB3 0HA, UK}

